Self-Supervised Real-time Video Stabilization

Videos are a popular media form, where online video streaming has recently gathered much popularity. In this work, we propose a novel method of real-time video stabilization - transforming a shaky video to a stabilized video as if it were stabilized via gimbals in real-time. Our framework is trainable in a self-supervised manner, which does not require data captured with special hardware setups (i.e., two cameras on a stereo rig or additional motion sensors). Our framework consists of a transformation estimator between given frames for global stability adjustments, followed by scene parallax reduction module via spatially smoothed optical flow for further stability. Then, a margin inpainting module fills in the missing margin regions created during stabilization to reduce the amount of post-cropping. These sequential steps reduce distortion and margin cropping to a minimum while enhancing stability. Hence, our approach outperforms state-of-the-art real-time video stabilization methods as well as offline methods that require camera trajectory optimization. Our method procedure takes approximately 24.3 ms yielding 41 fps regardless of resolution (e.g., 480p or 1080p).

==> section/discussion.tex <==
\section{Discussion}
%- When applying our real-time method on actual video streaming, if $M=30$ and $N=30$, the stabilized video will have a processing `lag' of 30 frames.
%\jaesik{Because there is lagging, it might be dangerous to say the method is good for online streaming. How about change our statement to be real-time stabilization?}
%\jinsoo{Don't mention lagging?}
%, meaning, the stabilized video will be 30 frames late than the streaming video.
%- Wang \etal~\shortcite{wang2018deep} and Xu \etal~\shortcite{xu2018deep} also have a processing lag of 29 (or 31) frames which are required as inputs.
%- Lagging process is not a crucial issue, especially if it is as small as 1 second (for 30 fps).
%- However, our method does possess the option to reduce this lag if needed, by reducing the window sizes $M$ and $N$ without noticeable loss in stability (shown in the ablation study of Sec.~\ref{ablation}).
%- On the other hand, the processing lag is fixed for methods of Wang \etal~\shortcite{wang2018deep} and Xu \etal~\shortcite{xu2018deep} since its deep networks require such frame inputs.
%- Because of this reason, Wang \etal~\shortcite{wang2018deep} and Xu \etal~\shortcite{xu2018deep} is unable to produce a stabilized video for the first 29 (or 31) input frames.
%- In contrast, as explained in Sec.~\ref{testing}, our method enables producing stabilized frames for the first (and last) 30 frames by dynamically reducing the window sizes to use available neighboring frames.

%- slight blur caused by the bilinear interpolation (PyTorch implementation)
%- Due to dealing with subpixel resolution
%- nearest-neighbor interpolation causes edge distortion
%- image processing level limitation (out of scope)
%- unnoticeable, better than baselines


Our approach provides the flexibility to enlarge the window size parameters for stronger video stability.
The window sizes can also be reduced to further improve computational speed without compromising much performance, as shown in the ablation study of Sec.~\ref{ablation}.
In contrast, the option of adjusting window size is absent in the works of  Wang \etal~\shortcite{wang2018deep} and Xu \etal~\shortcite{xu2018deep} that have a fixed processing window (due to their deep architecture design).
Because of this, Wang \etal~\shortcite{wang2018deep} and Xu \etal~\shortcite{xu2018deep} are unable to produce a stabilized video for the first 29 (or 31) input frames.
On the other hand, as explained in Sec.~\ref{testing}, our method enables producing stabilized frames for the first (and last) 30 frames by dynamically reducing the window sizes to use available neighboring frames.

A future direction of our work can be exploring different weighting schemes within the processing window or dynamically determining the window sizes for different stabilization effects.
Achieving this online is a challenging task since it must infer future movements or content.

\begin{figure}
    \includegraphics[width=1\linewidth,keepaspectratio]{Figures/failcase}
    \caption{Failure cases on severe camera movements including running and quick rotation scenes.}
    \label{failcase}
\end{figure}
